KODA: Kinematics--Observation Data Alignment for Humanoid Learning from Human Egocentric Demonstration

Training humanoid whole-body vision-language-action (VLA) policies requires costly robot demonstrations with aligned robot-view observations and controller-compatible whole-body state-action labels. Egocentric human demonstrations offer scalable supervision but have misaligned views and sparse motion cues. Existing approaches either pretrain policies that still require robot data for adaptation or generate controller-specific commands that limit reuse. Conversion also requires robot-view observations aligned with the generated whole-body motion. We present KODA (Kinematics-Observation Data Alignment), which converts egocentric RGB demonstrations into whole-body VLA training data using a reusable canonical trajectory to guide robot-view synthesis and generate controller-specific whole-body state-action supervision. KODA first generates a simulator-checked whole-body trajectory using a sparse tracker with sampling-based command optimization. This generated trajectory directly determines the onboard camera poses used to synthesize corresponding robot-view observations. The motion, observations, and task instruction form a canonical record. For each deployment controller, KODA optimizes commands to track the stored motion and records the corresponding action labels and proprioceptive states. When switching controllers, KODA retains this canonical record and regenerates whole-body state-action supervision for co-training with matching robot demonstrations. We evaluate KODA on four Unitree G1 loco-manipulation tasks using two whole-body controllers, SONIC and HEFT. With robot data held fixed, macro-average success on conditions covered by human demonstrations but absent from robot data improves by 45.0 and 46.25 percentage points, respectively. Under both controllers, this metric shows an upward trend across the evaluated human-data budgets, suggesting potential for further scaling.

==> B-migrated/abstract.tex <==
\begin{abstract}
Training humanoid whole-body vision--language--action (VLA) policies requires
costly robot demonstrations with aligned robot-view observations and
controller-compatible whole-body state--action labels. Egocentric human
demonstrations offer scalable supervision but have misaligned views and
sparse motion cues. Existing approaches either pretrain policies that still
require robot data for adaptation or generate controller-specific commands
that limit reuse. Conversion also requires robot-view observations aligned
with the generated whole-body motion. We present KODA
(Kinematics--Observation Data Alignment), which converts egocentric RGB
demonstrations into whole-body VLA training data using a reusable canonical
trajectory to guide robot-view synthesis and generate controller-specific
whole-body state--action supervision. KODA first generates a
simulator-checked whole-body trajectory using a sparse tracker with
sampling-based command optimization. This generated trajectory directly
determines the onboard camera poses used to synthesize corresponding
robot-view observations. The motion, observations, and task instruction form
a canonical record. For each deployment controller, KODA optimizes commands
to track the stored motion and records the corresponding action labels and
proprioceptive states. When switching controllers, KODA retains this
canonical record and regenerates whole-body state--action supervision for
co-training with matching robot demonstrations. We evaluate KODA on four
Unitree G1 loco-manipulation tasks using two whole-body controllers, SONIC
and HEFT. With robot data held fixed, macro-average success on conditions
covered by human demonstrations but absent from robot data improves by
45.0 and 46.25 percentage points, respectively. Under both controllers, this
metric shows an upward trend across the evaluated human-data budgets,
suggesting potential for further scaling.
\end{abstract}



\begin{IEEEkeywords}
% Index Terms—Learn from Human, Robotic Data Generation,
% Humanoid Lo-manipulation
Egocentric Human Video, Embodiment Alignment, Humanoid Loco-Manipulation
\end{IEEEkeywords}

